Discrepancy-Guided Reconstruction Learning for Image Forgery Detection

In this paper, we propose a novel image forgery detection paradigm for boosting the model learning capacity on both forgery-sensitive and genuine compact visual patterns. Compared to the existing methods that only focus on the discrepant-specific patterns (\eg, noises, textures, and frequencies), our method has a greater generalization. Specifically, we first propose a Discrepancy-Guided Encoder (DisGE) to extract forgery-sensitive visual patterns. DisGE consists of two branches, where the mainstream backbone branch is used to extract general semantic features, and the accessorial discrepant external attention branch is used to extract explicit forgery cues. Besides, a Double-Head Reconstruction (DouHR) module is proposed to enhance genuine compact visual patterns in different granular spaces. Under DouHR, we further introduce a Discrepancy-Aggregation Detector (DisAD) to aggregate these genuine compact visual patterns, such that the forgery detection capability on unknown patterns can be improved. Extensive experimental results on four challenging datasets validate the effectiveness of our proposed method against state-of-the-art competitors.

==> arxiv-Discrepancy-Guided Reconstruction Learning for Image Forgery Detection/Table1.tex <==
% Please add the following required packages to your document preamble:
\begin{table*}[t] 
\small
\centering
\setlength{\tabcolsep}{8pt}{% 列间距
\renewcommand\arraystretch{1.1}
\begin{tabular}{r|c|cccccccccc}
\toprule
\multirow{2}{*}{Methods}  & \multirow{2}{*}{Pub./Year} & \multicolumn{2}{c}{FF++ HQ} & \multicolumn{2}{c}{FF++ LQ} & \multicolumn{2}{c}{Celeb-DF} & \multicolumn{2}{c}{WLD} & \multicolumn{2}{c}{DFDC}  \\  \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}  
&   & \multicolumn{1}{c}{ACC } & \multicolumn{1}{c}{AUC } & \multicolumn{1}{c}{ACC } & \multicolumn{1}{c}{AUC } & \multicolumn{1}{c}{ACC } & \multicolumn{1}{c}{AUC } & \multicolumn{1}{c}{ACC } & \multicolumn{1}{c}{AUC } & \multicolumn{1}{c}{ACC } & \multicolumn{1}{c}{AUC } \\ \midrule
Xception   & ICCV'19 & 95.73 & 96.30 & 86.86 & 89.30 & 97.90  &  99.73  & 77.25 &  86.76  & 79.35 & 89.50   \\
Two branch & ECCV'20 & 96.43 & 98.70 & 86.34 & 86.59 &  –  &   –  &  – &   –  & – & –    \\
Add-Net    & ACM MM'20   & 96.78 & 97.74 & 87.50 & 91.01 & 96.93  &  99.55  & 76.25 &  86.17  & 78.71 & 89.85     \\
F$^3$-Net  & ECCV'20 & 97.52 & 98.10 & \textcolor{blue}{90.43} & 93.30 & 95.95  &  98.93  & 80.66 &  87.53  & 76.17 & 88.39     \\
SPSL       & CVPR'21 & 91.50 & 95.32 & 81.57 & 82.82 &  –  &   –  &  – &   –  & – & –    \\
RFM        & CVPR'21 & 95.69 & 98.79 & 87.06 & 89.83 & 97.96  &  \textcolor{green}{99.94}  & 77.38 &  83.92  & \textcolor{blue}{80.83} & 89.75     \\
Freq-SCL   & CVPR'21 & 96.69 & 99.28 & 89.00 & 92.39 &  –  &   –  &  – &   –  & – & –    \\
MAT   & CVPR'21 & \textcolor{blue}{97.60} & 99.29 & 88.69 & 90.40 & 97.92  &  \textcolor{green}{99.94}  & 82.86 &  90.71  & 76.81 & \textcolor{blue}{90.32}   \\
RECCE      & CVPR'22 & 97.06 & \textcolor{blue}{99.32} & \textcolor{green}{91.03} & \textcolor{green}{95.02} & \textcolor{green}{98.59}  &  \textcolor{green}{99.94}  & \textcolor{blue}{83.25} &  \textcolor{green}{92.02}  & \textcolor{green}{81.20} & \textcolor{green}{91.33}    \\
ITA-SIA        & ECCV'22 & \textcolor{green}{97.64} & \textcolor{green}{99.35} & 90.23 & \textcolor{blue}{93.45} & \textcolor{blue}{98.48}  &  \textcolor{red}{99.96}  & \textcolor{green}{83.95} &  \textcolor{blue}{91.34}  &  – &  –    \\

\rowcolor{ours}
DisGRL & IJCAI'23 &  \textcolor{red}{97.69} &  \textcolor{red}{99.48} & \textcolor{red}{91.27} & \textcolor{red}{95.19} & \textcolor{red}{98.71}  &  \textcolor{blue}{99.91} & \textcolor{red}{84.53} &  \textcolor{red}{93.27}  & \textcolor{red}{82.35} & \textcolor{red}{92.50}    \\
\bottomrule                       
\end{tabular}}
\vspace{-2mm}
\caption{Intra-dataset evaluation and result comparisons on four benchmarks. ``HQ'' and ``LQ'' denote the High-Quality version and the Low-Quality version of the corresponding dataset, respectively.
The top three results are highlighted in \textcolor{red}{red}, \textcolor{green}{green}, and \textcolor{blue}{blue}, respectively.}
\label{table:1}
\vspace{-2mm}
\end{table*}




==> arxiv-Discrepancy-Guided Reconstruction Learning for Image Forgery Detection/Table2.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[t] 
\small
\centering
\setlength{\tabcolsep}{4.5pt}{ 
\renewcommand\arraystretch{1.1}
\begin{tabular}{r|cccccc}
\toprule
\multirow{2}{*}{Methods}  &  \multicolumn{2}{c}{Celeb-DF} & \multicolumn{2}{c}{WLD} & \multicolumn{2}{c}{DFDC}  \\  \cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7}  
&  \multicolumn{1}{c}{AUC  $\uparrow$} & \multicolumn{1}{c}{EER $\downarrow$} & \multicolumn{1}{c}{AUC  $\uparrow$} & \multicolumn{1}{c}{EER $\downarrow$} & \multicolumn{1}{c}{AUC $\uparrow$} & \multicolumn{1}{c}{EER $\downarrow$}   \\ \midrule
Xception   & 61.80 & 41.73 & 62.72 & 40.65 & 63.61  & 40.58  \\
F$^3$-Net  & 61.51   & 42.03 & 57.10 & 45.12 & 64.60 & 39.84  \\
Add-Net    & 65.29 & 38.90 & 62.35 & 41.42 & 64.78 & 40.23  \\
RFM        & 65.63 & 38.54 & 57.75 & 45.45 & 66.01 & 39.05    \\
MAT   & 67.02 & 37.90 & 59.74 & 43.73 & 68.01 & 37.17  \\
RECCE      & 68.71 & 35.73 & 64.31 & 40.53 & 69.06 & 36.08  \\
\rowcolor{ours}
DisGRL      & \textbf{70.03} &  \textbf{34.23} &  \textbf{66.73} & \textbf{39.24} & \textbf{70.89} & \textbf{34.27}   \\
\bottomrule                       
\end{tabular}
\vspace{-2mm}
\caption{Cross-dataset result evaluation on FF++ (LQ), Celeb-DF, WLD, and DFDC in terms of AUC (\%) and EER (\%).}
\label{table:2}}
\vspace{-3mm}
\end{table}




==> arxiv-Discrepancy-Guided Reconstruction Learning for Image Forgery Detection/Table3.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[t] 
\small
%\centering
\setlength{\tabcolsep}{5.5pt}{ % 列间距
\renewcommand\arraystretch{1.1}
\begin{tabular}{r|cccccc}
\toprule
Methods & Train & DF   &  F2F    &  FS   &  NT   &  CAvg.
\\ \midrule
Freq-SCL &  \multirow{4}{*}{DF} & \cellcolor[gray]{.95}98.91 & 58.90 &66.87 &63.61& 63.13 \\
MAT &   & \cellcolor[gray]{.95}99.51 & 66.41 & 67.33 & 66.01 & 66.58 \\
RECCE &   & \cellcolor[gray]{.95}99.65 & 70.66 & 74.29 & 67.34 & 70.76 \\
DisGRL &   & \cellcolor[gray]{.95}{\textbf{99.67}}   & \textbf{71.76}   &  \textbf{75.21} & \textbf{68.74}  &  \textbf{71.90}  \\  \midrule

Freq-SCL &  \multirow{4}{*}{F2F} & 67.55 &\cellcolor[gray]{.95}93.06 & 55.35 & 66.66 & 63.19 \\
MAT &   & 73.04 &\cellcolor[gray]{.95}97.96 & 65.10 & 71.88 & 70.01 \\
RECCE &      & \textbf{75.99} &\cellcolor[gray]{.95}98.06 & 64.53 & 72.32 & 70.95 \\
DisGRL &         &  75.73   &\cellcolor[gray]{.95}\textbf{98.69}       &  \textbf{65.71}    &   \textbf{74.15}    &  \textbf{71.86}     \\  \midrule

Freq-SCL &  \multirow{4}{*}{FS} & 75.90 &54.64 &\cellcolor[gray]{.95}98.37 &49.72& 60.09 \\
MAT &   & 82.33 &61.65 &\cellcolor[gray]{.95}98.82 &54.79& 66.26 \\
RECCE &   & 82.39 &64.44 &\cellcolor[gray]{.95}98.82 &56.70& 67.84 \\
DisGRL &   & \textbf{82.73} & \textbf{64.85}  &\cellcolor[gray]{.95}{\textbf{99.01}} & \textbf{56.96} & \textbf{68.18}  \\  \midrule

Freq-SCL &  \multirow{4}{*}{NT} & 79.09 & 74.21 & 53.99 &\cellcolor[gray]{.95}88.54 & 69.10 \\
MAT &   & 74.56 & 80.61 & 60.90 &\cellcolor[gray]{.95}93.34 & 72.02 \\
RECCE &   & 78.83 & 80.89 & 63.70 &\cellcolor[gray]{.95}93.63 & 74.47 \\
DisGRL &   & \textbf{80.29} & \textbf{83.30} & \textbf{65.23}  &\cellcolor[gray]{.95}{\textbf{94.10}} & \textbf{76.27} \\  
\bottomrule                       
\end{tabular}
\vspace{-2mm}
\caption{Cross-manipulation evaluation in terms of AUC (\%). Diagonal results indicate intra-domain performance. DeepFakes (DF), Face2Face (F2F), FaceSwap (FS), and NeuralTextures (NT) are four image manipulation approaches in FF++~\protect\cite{rossler2019faceforensics++}. ``CAvg.'' denotes the average of cross-manipulation evaluations.}
\label{table:3}}
\vspace{-2mm}
\end{table}


  

==> arxiv-Discrepancy-Guided Reconstruction Learning for Image Forgery Detection/Table4.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[t] 
\footnotesize
\setlength{\tabcolsep}{3.2pt}{ % 列间距
%\renewcommand\arraystretch{1.2} % 行间距
%\resizebox{\textwidth}{!}{
\begin{tabular}{r|cccccccc}
\toprule
\multirow{2}{*}{Methods}  & \multicolumn{2}{c}{GID-DF} & \multicolumn{2}{c}{GID-F2F} & \multicolumn{2}{c}{GID-FS} & \multicolumn{2}{c}{GID-NT}  \\  \cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} \cmidrule(l){8-9}
&    \multicolumn{1}{c}{ACC } & \multicolumn{1}{c}{AUC } & \multicolumn{1}{c}{ACC } & \multicolumn{1}{c}{AUC } & \multicolumn{1}{c}{ACC } & \multicolumn{1}{c}{AUC } & \multicolumn{1}{c}{ACC } & \multicolumn{1}{c}{AUC } \\ \midrule
Multi-task   &  66.8 & – & 56.5 & – & 51.7  &  –  & 56.0 &  –    \\
MLDG         &  67.2 & 73.1 & 58.1 & 61.7  & 58.1   & 61.7  & 56.9 &  60.7     \\
LTW          &  69.1 & 75.6 & 65.7 & 72.4 & 62.5  &  68.1  & 58.5 &  60.8     \\
DCL          &  75.9 & 83.8 & 67.9 & 75.1 & –  &  –  & – &  –     \\
\rowcolor{ours}
DisGRL         & \textbf{77.3}       & \textbf{86.1}      & \textbf{75.8}      &    \textbf{84.3}   &   \textbf{76.9}     &   \textbf{86.3}      &  \textbf{66.3}  & \textbf{72.8}      \\
\bottomrule                       
\end{tabular}}
\vspace{-2mm}
\caption{Multi-source manipulation evaluation in terms of ACC (\%) and AUC (\%). The protocols and results are from LTW~\protect\cite{sun2021domain} and DCL~\protect\cite{sun2022dual}.}
\label{table:4}
\vspace{-2mm}
\end{table}




==> arxiv-Discrepancy-Guided Reconstruction Learning for Image Forgery Detection/Table5.tex <==
\begin{table}[t] 
\centering
\footnotesize
\setlength{\tabcolsep}{4.5pt}{ % 列间距
\renewcommand\arraystretch{1.1} % 行间距
\begin{tabular}{c|ccccc|cc}
\toprule
NO & Baseline  & {Rec}-1 & {Rec}-2 & DEA & RFA & ACC & AUC \\ 
 \midrule
a) & \checkmark &   &  &  &  & 77.13 & 86.21    \\%\cdashline{1-7}[0.5pt/2pt]
b) & \checkmark  &  \checkmark  &  &  &   & 80.76  & 88.47  \\
c) & \checkmark  &    &\checkmark  &  &   & 81.37  & 88.94  \\
d) &\checkmark  &  \checkmark  &  \checkmark &  &  & 82.84 & 90.98\\
e) &\checkmark   &  \checkmark  &  \checkmark & \checkmark &  & 83.68 & 92.35   \\
f) &\checkmark   &  \checkmark  &  \checkmark &  & \checkmark & 83.24 & 91.68  \\
g) & \checkmark   &    \checkmark    &   \checkmark     &    \checkmark &     \checkmark   &   \textbf{84.53}     & \textbf{93.27}   \\
\bottomrule                       
\end{tabular}}
\vspace{-2mm}
\caption{Ablation studies on WildDeepfake~\protect\cite{wilddeepfake} in terms of ACC (\%) and AUC (\%). ``RFA'' and ``DEA'' are the Reconstruction-guidance Feature Aggregation module and Discrepancy External Attention (DEA) block, respectively. }
\label{table:5}
\end{table}

==> arxiv-Discrepancy-Guided Reconstruction Learning for Image Forgery Detection/Table6.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[ht] 
\footnotesize
\setlength{\tabcolsep}{3.2pt}{ % 列间距
%\renewcommand\arraystretch{1.2} % 行间距
%\resizebox{\textwidth}{!}{
\begin{tabular}{r|cccccccc}
\toprule
\multirow{2}{*}{Methods}  & \multicolumn{2}{c}{GID-DF} & \multicolumn{2}{c}{GID-F2F} & \multicolumn{2}{c}{GID-FS} & \multicolumn{2}{c}{GID-NT}  \\  \cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7} \cmidrule(l){8-9}
&    \multicolumn{1}{c}{ACC } & \multicolumn{1}{c}{AUC } & \multicolumn{1}{c}{ACC } & \multicolumn{1}{c}{AUC } & \multicolumn{1}{c}{ACC } & \multicolumn{1}{c}{AUC } & \multicolumn{1}{c}{ACC } & \multicolumn{1}{c}{AUC } \\ \midrule
Multi-task   &  70.3 & – & 58.7 & – & 49.7  &  –  & 60.3 &  –    \\
MLDG         &  84.2 & 91.8 & 63.4 & 77.1  & 52.7   & 60.9  & 62.1 &  78.0     \\
LTW          &  85.6 & 92.7 & 65.6 & 80.2 & 54.9  &  64.0  & 65.3 &  77.3     \\
DCL          &  87.7 & 94.9 & 68.4 & 82.9 & –  &  –  & – &  –     \\
\rowcolor{ours}
DisGRL         & \textbf{88.3}       & \textbf{95.7}      & \textbf{74.7}      &    \textbf{89.4}   &   \textbf{58.4}     &   \textbf{67.9}      &  \textbf{67.6}  & \textbf{84.6}      \\
\bottomrule                       
\end{tabular}}
%}
\caption{Multi-source manipulation evaluation in terms of ACC (\%) and AUC (\%). The protocols and results are from LTW~\protect\cite{sun2021domain} and DCL~\protect\cite{sun2022dual}. GID-DF indicates training on the remaining three facial manipulation techniques of FF++ (HQ) and testing on DeepFakes class. The same for the other setting.}
\label{table:6}
\end{table}

==> arxiv-Discrepancy-Guided Reconstruction Learning for Image Forgery Detection/Table7.tex <==
\begin{table}[h!] 
%\vspace{-3mm}
\small
\centering
\footnotesize
\setlength{\tabcolsep}{0.9pt}{ % 列间距
%\renewcommand\arraystretch{.7} % 行间距
\begin{tabular}{l|cccc}
\toprule
Methods & Inference time  & Training time & \textcolor{gray}{Params}  & \textcolor{gray}{FLOPs}   \\ 
 \midrule
RECCE    & 29.7ms & 33.5mins  & \textcolor{gray}{30.07M} & \textcolor{gray}{15.11G}   \\%\cdashline{1-7}[0.5pt/2pt]
LTW    & 23.5ms & 17.9mins  & \textcolor{gray}{98.78M} & \textcolor{gray}{63.25G}   \\%\cdashline{1-7}[0.5pt/2pt]
MVSS-Net  & 21.9ms & 19.4mins  & \textcolor{gray}{146.81M} & \textcolor{gray}{67.94G}   \\%\cdashline{1-7}[0.5pt/2pt]
\textbf{DisGRL(w/o Rec-2)}  & 15.4ms & 8.4mins & \textcolor{gray}{89.72M}  & \textcolor{gray}{54.86G}\\
\textbf{DisGRL(w/o Rec-1)}   & 16.5ms & 9.2mins & \textcolor{gray}{82.34M}  & \textcolor{gray}{48.05G} \\
\textbf{DisGRL}   & 20.7ms & 10.1mins  & \textcolor{gray}{95.87M}  &  \textcolor{gray}{58.09G}\\
\bottomrule                       
\end{tabular}}
%\vspace{-3mm}
\caption{Results are obtained on a single NVIDIA GeForce RTX 3090 GPU. The training time is the average over 10 epochs, and the inference time is the average of over 14,000 test images from FF++ (Neural Textures) dataset with image size 299 $\times$ 299. ``M'' denotes million, ``ms'' denotes milliseconds, and ``mins'' denotes minutes. }
\label{table:7}
%\vspace{-4mm}
\end{table}
